Time Series Classification via Topological Data Analysis

In this paper, we develop topological data analysis methods for classification tasks on univariate time series. As an application, we perform binary and ternary classification tasks on two public datasets that consist of physiological signals collected under stress and non-stress conditions. We accomplish our goal by using persistent homology to engineer stable topological features after we use a time delay embedding of the signals and perform a subwindowing instead of using windows of fixed length. The combination of methods we use can be applied to any univariate time series and in this application allows us to reduce noise and use long window sizes without incurring an extra computational cost. We then use machine learning models on the features we algorithmically engineered to obtain higher accuracies with fewer features.

==> Karan and Kaygun/figureCodes/Driver_LOSOCV_binary_table.tex <==
\begin{tabular}{@{}llclclc@{}}
\toprule
 &
  \multicolumn{1}{c}{} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Delay\\ Embeddings\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Level\\ Sets\end{tabular}} &
   \\ \cmidrule(lr){3-4}
\cmidrule(lr){5-6} &
  \multicolumn{1}{c}{Clf} &
  Acc &
  \multicolumn{1}{c}{Dgm} &
  Acc &
  \multicolumn{1}{c}{Dgm} &
  \begin{tabular}[c]{@{}c@{}}All\\ Dgms\end{tabular} \\ \midrule
ECG      & RF  & 65.74           & $2\fs$     & \highest{71.11} & Upper & 67.61           \\
EMG      & RF  & 79.54           & $1\fs,H0$  & 82.04           & Both & 79.91           \\
Foot GSR & RF  & 90.83           & $.5\fs$    & \highest{92.26} & Upper & 91.88           \\
Hand GSR & RF  & \highest{82.47} & $1\fs,H0$  & 78.75           & Upper & 81.44           \\
HR       & SVC & 73.83           & $1\fs$     & 71.06           & Both & \highest{74.67} \\
RESP     & RF  & 93.27           & $1\fs,H0$  & \highest{98.07} & Both & 95.54           \\ \midrule
All      & RF  & 94.96           & $.5\fs,H1$ & \highest{96.24} & Upper & 95.39           \\ \bottomrule
\end{tabular}

==> Karan and Kaygun/figureCodes/Driver_LOSOCV_ternary_table.tex <==
\begin{tabular}{@{}llclclc@{}}
\toprule
 &
  \multicolumn{1}{c}{} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Delay\\ Embeddings\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Level\\ Sets\end{tabular}} &
   \\ \cmidrule(lr){3-4}
\cmidrule(lr){5-6} &
  \multicolumn{1}{c}{Clf} &
  Acc &
  \multicolumn{1}{c}{Dgm} &
  Acc &
  \multicolumn{1}{c}{Dgm} &
  \begin{tabular}[c]{@{}c@{}}All\\ Dgms\end{tabular} \\ \midrule
ECG      & RF  & 53.32           & $2\fs,H1$  & \highest{58.49} & Upper & 56.68           \\
EMG      & RF  & 66.87           & $.5\fs$    & \highest{69.14} & Upper & 66.49           \\
Foot GSR & RF  & 79.30           & $.5\fs$    & 79.60           & Both & \highest{80.08} \\
Hand GSR & RF  & \highest{67.26} & $2\fs,H0$  & 65.42           & Upper & 65.80           \\
HR       & SVC & 59.30           & $1\fs,H1$  & 59.80           & Both & \highest{60.61} \\
RESP     & SVC & 81.28           & $.5\fs$    & 85.71           & Both & \highest{85.81} \\ \midrule
All      & SVC & 82.50           & $.5\fs,H1$ & \highest{85.15} & Both & 80.59           \\ \bottomrule
\end{tabular}

==> Karan and Kaygun/figureCodes/Wesad_LOSOCV_binary_table.tex <==
\begin{tabular}{@{}llclclcc@{}}
\toprule
 &
  \multicolumn{1}{c}{} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Delay\\ Embeddings\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Level\\ Sets\end{tabular}} &
   &
   \\ \cmidrule(lr){3-4}
\cmidrule(lr){5-6} &
  \multicolumn{1}{c}{Clf} &
  Acc &
  \multicolumn{1}{c}{Dgm} &
  Acc &
  \multicolumn{1}{c}{Dgm} &
  \begin{tabular}[c]{@{}c@{}}All\\ Dgms\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Original\\ Findings\end{tabular} \\ \midrule
\textit{Chest}    & \multicolumn{1}{c}{} &                 & \multicolumn{1}{c}{} &       & \multicolumn{1}{c}{} &                 &                 \\
\hspace{2mm} ACC  & RF                   & \highest{87.69} & $.5\fs,H0$           & 84.82 & Both                    & 84.18           & 73.87           \\
\hspace{2mm} ECG  & LDA                  & \highest{88.70} & $1\fs,H0$            & 81.62 & Both                    & 85.23           & 85.44           \\
\hspace{2mm} EMG  & LDA                  & \highest{73.07} & $1\fs$               & 68.03 & Lower                    & 69.75           & 67.10           \\
\hspace{2mm} EDA  & LDA                  & 76.57           & $1\fs,H1$            & 81.55 & Lower                    & 81.49           & \highest{81.70} \\
\hspace{2mm} TEMP & SVC                  & \highest{70.19} & $.5\fs$              & 70.19 & Both                    & 68.07           & 69.49           \\
\hspace{2mm} RESP & LDA                  & 81.72           & $.5\fs$              & 87.75 & Both                    & \highest{90.10} & 88.09           \\ \midrule
\textit{Wrist}    &                      &                 &                      &       &                      &                 &                 \\
\hspace{2mm} ACC  & RF                   & 82.95           & $.5\fs$              & 82.81 & Both                    & \highest{83.52} & 71.69           \\
\hspace{2mm} BVP  & LDA                  & 85.21           & $1\fs$               & 72.51 & Lower                    & 84.03           & \highest{85.83} \\
\hspace{2mm} EDA  & RF                   & 81.19           & $2\fs$               & 84.01 & Upper                    & \highest{85.11} & 79.71           \\
\hspace{2mm} TEMP & RF                   & \highest{71.44} & $.5\fs$              & 70.00 & Both                    & 70.02           & 69.24           \\ \midrule
All chest         & SVC                  & 89.32           & $1\fs,H0$            & 91.97 & Lower                    & 91.79           & \highest{92.83} \\
All wrist         & SVC                  & \highest{88.77} & $2\fs$               & 87.04 & Lower                    & 88.55           & 87.12           \\
All               & SVC                  & 92.91           & $2\fs,H1$            & 92.95 & Both                    & \highest{94.46} & 92.28           \\ \bottomrule
\end{tabular}

==> Karan and Kaygun/figureCodes/Wesad_LOSOCV_ternary_table.tex <==
\begin{tabular}{@{}llclclcc@{}}
\toprule
 &
  \multicolumn{1}{c}{} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Delay\\ Embeddings\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Level\\ Sets \end{tabular}} &
   &
   \\ \cmidrule(lr){3-4}
\cmidrule(lr){5-6} &
  \multicolumn{1}{c}{Clf} &
  Acc &
  \multicolumn{1}{c}{Dgm} &
  Acc &
  \multicolumn{1}{c}{Dgm} &
  \begin{tabular}[c]{@{}c@{}}All\\ Dgms\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Original\\ Findings\end{tabular} \\ \midrule
\textit{Chest}    & \multicolumn{1}{c}{} &                 & \multicolumn{1}{c}{} &       & \multicolumn{1}{c}{} &                 &                 \\
\hspace{2mm} ACC  & SVC                  & 72.34           & $2\fs$               & 69.77 & Upper                    & \highest{74.47} & 56.56           \\
\hspace{2mm} ECG  & SVC                  & \highest{76.27} & $1\fs$               & 66.11 & Upper                    & 72.72           & 66.29           \\
\hspace{2mm} EMG  & SVC                  & 59.00           & $1\fs$               & 54.64 & Both                    & \highest{59.67} & 53.99           \\
\hspace{2mm} EDA  & LDA                  & 66.31           & $.5\fs,H0$           & 66.56 & Upper                    & \highest{70.03} & 67.07           \\
\hspace{2mm} TEMP & LDA                  & 54.75           & $1\fs,H1$            & 53.02 & Upper                    & 48.92           & \highest{55.68} \\
\hspace{2mm} RESP & SVC                  & 68.46           & $2\fs$               & 70.73 & Both                    & \highest{75.57} & 72.37           \\ \midrule
\textit{Wrist}    &                      &                 &                      &       &                      &                 &                 \\
\hspace{2mm} ACC  & RF                   & 68.02           & $.5\fs$              & 67.28 & Upper                    & \highest{68.65} & 57.20           \\
\hspace{2mm} BVP  & SVC                  & 71.64           & $1\fs$               & 60.67 & Lower                    & \highest{73.41} & 70.17           \\
\hspace{2mm} EDA  & RF                   & 69.23           & $2\fs$               & 70.50 & Both                    & \highest{72.07} & 62.32           \\
\hspace{2mm} TEMP & LDA                  & 55.87           & .$5\fs$              & 54.79 & Upper                    & 54.93           & \highest{58.96} \\ \midrule
All chest         & SVC                  & \highest{78.85} & $1\fs,H0$            & 75.34 & Upper                    & 77.96           & 76.50           \\
All wrist         & RF                   & 73.93           & $2\fs$               & 71.94 & Upper                    & 74.72           & \highest{75.21} \\
All               & SVC                  & 80.63           & $1\fs$               & 80.56 & Lower                    & \highest{81.35} & 79.57           \\ \bottomrule
\end{tabular} 


==> Karan and Kaygun/figureCodes/filtration.tex <==
\begin{subfigure}{0.23\textwidth} 
\includegraphics[trim={1cm 0cm 1cm 0cm},clip, scale=.27]{growing_epsilon_0.03} \caption{$\varepsilon = .0$} \end{subfigure}
\begin{subfigure}{0.23\textwidth} 
\includegraphics[trim={1cm 0cm 1cm 0cm},clip, scale=.27]{growing_epsilon_0.15} \caption{$\varepsilon = .15$} \end{subfigure}
\begin{subfigure}{0.23\textwidth} 
\includegraphics[trim={1cm 0cm 1cm 0cm},clip, scale=.27]{growing_epsilon_0.18} \caption{$\varepsilon = .18$} \end{subfigure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[trim={1cm 0cm 1cm 0cm},clip, scale=.27]{growing_epsilon_0.34} \caption{$\varepsilon = .34$} \end{subfigure}

==> Karan and Kaygun/figureCodes/timeseries.tex <==
\begin{subfigure}{0.45\textwidth} 
\centering
\includegraphics[width = 5cm]{timeseries_sine} \caption{Noisy time series from $y=\sin x$.} \end{subfigure}
\begin{subfigure}{0.45\textwidth} 
\centering
\includegraphics[width = 5cm]{timeseries_sine5} \caption{Noisy time series from $y=\sin^5 x$.} \end{subfigure}

\begin{subfigure}{.22\textwidth} 
\centering
\includegraphics[width = 2.2cm]{timeseries_pca_sine_15dim} \caption{$d=15$} \end{subfigure}
\begin{subfigure}{.22\textwidth} 
\centering
\includegraphics[width = 2.2cm]{timeseries_pca_sine_50dim} \caption{$d=50$} \end{subfigure}
\begin{subfigure}{0.22\textwidth} 
\centering
\includegraphics[width = 2.2cm]{timeseries_pca_sine5_15dim} \caption{$d=15$} \end{subfigure}
\begin{subfigure}{0.22\textwidth} 
\centering
\includegraphics[width = 2.2cm]{timeseries_pca_sine5_50dim} \caption{$d=50$} \end{subfigure}
